GRID: Scene-Graph-based Instruction-driven Robotic Task Planning

Recent works have shown that Large Language Models (LLMs) can facilitate the grounding of instructions for robotic task planning. Despite this progress, most existing works have primarily focused on utilizing raw images to aid LLMs in understanding environmental information. However, this approach not only limits the scope of observation but also typically necessitates extensive multimodal data collection and large-scale models. In this paper, we propose a novel approach called Graph-based Robotic Instruction Decomposer (GRID), which leverages scene graphs instead of images to perceive global scene information and iteratively plan subtasks for a given instruction. Our method encodes object attributes and relationships in graphs through an LLM and Graph Attention Networks, integrating instruction features to predict subtasks consisting of pre-defined robot actions and target objects in the scene graph. This strategy enables robots to acquire semantic knowledge widely observed in the environment from the scene graph. To train and evaluate GRID, we establish a dataset construction pipeline to generate synthetic datasets for graph-based robotic task planning. Experiments have shown that our method outperforms GPT-4 by over 25.4% in subtask accuracy and 43.6% in task accuracy. Moreover, our method achieves a real-time speed of 0.11s per inference. Experiments conducted on datasets of unseen scenes and scenes with varying numbers of objects demonstrate that the task accuracy of GRID declined by at most 3.8%, showcasing its robust cross-scene generalization ability. We validate our method in both physical simulation and the real world. More details can be found on the project page https://jackyzengl.github.io/GRID.github.io/.

==> data_generation.tex <==
% \subsubsection{Dataset Generation}\label{subsubsection-data-generation}

% graph node edge可扩展
To generate data, we constructed a dictionary including various node types, edge types, and their respective properties. The advantage of synthesizing the dataset with an algorithm is that nodes, edges, actions, and instructions can be easily managed. Simply by changing the content in the dictionary, the depicted scene in the graph can be altered. Currently, our emphasis is on generating domestic scenes. Thus, the nodes are the rooms and objects that are commonly found in houses.


% How we generate scene 0
We start by establishing a scene graph at state 0. Initially, a floor node is created as the foundational element of the scene hierarchy. Subsequently, we attach room nodes to the root node. This is done by randomly sampling a distinct set of room nodes from the dictionary, with the connecting edge between room nodes and the floor node signifying an \texttt{in} relationship. Currently, the scenario of a room inside another room is excluded. Finally, a selection of objects is randomly drawn from the dictionary. These selected objects, known as scene objects, are integrated into the scene. Their locations are defined in relation to rooms or other objects. The former indicates a relationship of \texttt{in}, and the latter depicts a \texttt{on} relationship, suggesting the act of stacking. 

% How we generate instruction-subtask
Once the scene graph for state 0 is established, the entire scene is viewed as a blueprint. From this, we generate a list of instructions and associated subtask pairs suitable for the scene. 
A range of subtask sequences that the robot can execute are predefined as shown in Tab. \ref{tab-Subtask_Action_Count}. The corresponding instructions come in various expressive forms. Multiple expressions of the same instruction were generated using ChatGPT-4, which served as an instruction template. After selecting an instruction-subtask pair, we extract an instruction expression from the templates, then incorporate the names of the source and target objects into both the instruction templates and the subtask sequence. 
% instruction, subtask 可扩展
Tab. \ref{tab-instruction-subtask-examples} showcases examples of these instruction-subtask combinations. It's worth noting that both the instruction templates and subtasks are adaptable, enabling modifications based on a robot's capabilities.

% How to update scene and robot accordingly 
In practical scenarios, subtasks are the decision of the robot after viewing the scene graph and robot graph. As such, the synthesized subtasks serve as guidelines in the generation of robot and scene graphs across varying states. 
For example, when the robot is at the state shown in Fig. \ref{fig-First_Pic}, after successfully executing the subtask GRID generated which is to pick up the teacup, the robot should have the teacup in its hand. Thus, the updated robot graph should have a cup with a \texttt{grasp} relationship, and the node should also be removed from the updated scene graph.
For instance, referring to Fig. \ref{fig-First_Pic}, the current predicted subtask is pick tea cup 46. Consequently, the updated robot graph should depict the cup with a "grasp" relationship, and the teacup node should also be removed from the refreshed scene graph.


==> figure/dataset_statistics/Relationship_description_table.tex <==
\begin{table}[h]
        \centering
	\begin{tabular}{ lp{5cm} }
		\hline
		\textbf{Relationship} & \textbf{Definition} \\
		\hline
		in & target object is in source object \\
		
		on & target object is on top of source object \\

		beside & target object and source object are in the same parent object, 
		the Euclidean distance between their 6DoF positions are less than one metre apart,
		target object is the closest object to the source object, while they do not have 'in' or 'on' relationships.
		\\
		
		grasp & target object is grasped by the source object \\
		\hline
	\end{tabular}
	\caption{The type of edges in the graph and their definitions. More other relationships can be added if it is needed to be used in more complex scenes.}
	\label{tab edge definition}
\end{table}


==> figure/dataset_statistics/instr-subtask-pair-table.tex <==
\begin{table*}[t]
    \centering
	\begin{tabular}{ llp{0.2\textwidth} }
        \hline
        \textbf{Task Type} & \textbf{Instruction Example} & \textbf{Subtasks Example} \\
        \hline
        \multirow{3}{0.2\textwidth}{Move-Place-Finish} 
        &\multirow{3}{0.3\textwidth}{Please move to the green dining table and place the object there}
        & move 22 (dining table) \\
        & & place to 22 (dining table) \\
        & & finish 0 (floor)\\
        
        \hline
        %  pick place\_to finish
        \multirow{3}{0.2\textwidth}{Pick-Place-Finish}
        &\multirow{3}{0.3\textwidth}{Please pick up the tea cup and place it on the green dining table.}
        & pick 45 (tea cup)\\
        && place to 22 (dining table)\\
        && finish 0 (floor)\\
        \hline

        \multirow{3}{0.2\textwidth}{Move-Pick-Finish}
        &\multirow{3}{0.3\textwidth}{Can you please go to tea cup and pick it up?}
        & move 45 (tea cup)\\
        && pick 45 (tea cup)\\
        && finish 0 (floor)\\
        \hline

        \multirow{4}{0.2\textwidth}{Move-Pick-Place-Finish}
        &\multirow{4}{0.3\textwidth}{Move to tea cup, pick it up, then place it on the dining table.}
        & move 45 (tea cup)\\
        && pick 45 (tea cup)\\
        && place to 22 (dining table)\\
        && finish 0 (floor)\\
        \hline

        \multirow{4}{0.2\textwidth}{Pick-Move-Place-Finish}
        & \multirow{4}{0.3\textwidth}{Pick up the tea cup. Then, proceed towards dining table. Once there, place it.}
        & pick 45 (tea cup)\\
        && move 22 (dining table)\\
        && place to 22 (dining table)\\
        && finish 0 (floor)\\
        \hline

        \multirow{5}{0.2\textwidth}{Pick-Move-Place-Move-Finish}
        &\multirow{5}{0.3\textwidth}{Please pick up the tea cup, move to the dining table, place it there, then proceed to the kitchen.}
        & pick 45 (tea cup) \\
        && move 22 (dining table)\\
        && place to 22 (dining table)\\
        && move 1 (kitchen)\\
        && finish 0 (floor)\\
        \hline

        \multirow{5}{0.2\textwidth}{Move-Pick-Place-Move-Finish}
        &\multirow{5}{0.3\textwidth}{Could you first move to the tea cup, pick it up, then take it to the dining table and place it there? After doing so, please proceed to the kitchen.}
        & move 45 (tea cup)\\
        && pick 45 (tea cup)\\
        && place to 22 (dining table)\\
        && move 1 (kitchen)\\
        && finish 0 (floor)\\
        \hline

        \multirow{5}{0.2\textwidth}{Pick-Move-Place-Move-Pick-Finish}
        &\multirow{5}{0.3\textwidth}{Please pick up the tea cup, move to the dining table, and place it there. Then proceed to the kitchen.}
        & pick 45 (tea cup)\\
        && move dining table 11\\
        && place to 45 (tea cup)\\
        && move 1 (kitchen)\\
        && finish 0 (floor)\\
        \hline

        \multirow{6}{0.2\textwidth}{Place-Move-Pick-Move-Place-Finish}
        &\multirow{6}{0.3\textwidth}{Put the object at the dining table. Then go to the tea cup and pick it up. At the end, go to kitchen table and put it there.}
        & place to 22 (dining table)\\
        && move 45 (tea cup)\\
        && pick 45 (tea cup)\\
        && move 7 (kitchen table)\\
        && place to 7 (kitchen table)\\
        && finish 0 (floor)\\
        \hline



        % Revolute open/close
        \multirow{5}{0.2\textwidth}{Move-RevOpen-Pick-RevClose-Finish}
        &\multirow{5}{0.3\textwidth}{Please proceed to the fridge, open it up, grab the apple inside, then make sure to close it.}
        & move 35 (fridge)\\
        && revolute open 35 (fridge)\\
        && pick apple 30\\
        && revolute close 35 (fridge)\\
        && finish 0 (floor)\\
        \hline
        % longitudinal open/close
        \multirow{5}{0.2\textwidth}{Move-LongOpen-Pick-LongClose-Finish}
        &\multirow{5}{0.3\textwidth}{Please proceed to the draw, open it up, grab the tea cup inside, then make sure to close it.}
        & move 9 (draw)\\
        && longitudinal open 9 (draw)\\
        && pick 45 (tea cup)\\
        && longitudinal close 9 (draw)\\
        && finish 0 (floor)\\
        \hline

        \multirow{5}{0.2\textwidth}{Move-RevOpen-Place-RevClose-Finish}
        &\multirow{5}{0.3\textwidth}{Head to the fridge, open it up, place the object inside, and then secure it shut.}
        & move 35 (fridge)\\
        && revolute open 35 (fridge)\\
        && place to 35 (fridge)\\
        && revolute close 35 (fridge)\\
        && finish 0 (floor)\\
        \hline
        \multirow{5}{0.2\textwidth}{Move-LongOpen-Place-LongClose-Finish}
        &\multirow{5}{0.3\textwidth}{Head to the draw, open it up, place the object inside, and then secure it shut.}
        & move 9 (draw)\\
        && longitudinal open 9 (draw)\\
        && place to 9 (draw)\\
        && longitudinal close 9 (draw)\\
        && finish 0 (floor)\\
        \hline



        


        \multirow{6}{0.2\textwidth}{Move-RevOpen-Place-Revclose-Move-Finish}
        &\multirow{6}{0.3\textwidth}{Please head to the fridge, open it, place the object inside, close it, then proceed to the kitchen.}
        & move 35 (fridge)\\
        && revolute open 35 (fridge)\\
        && place to 35 (fridge)\\
        && revolute close 35 (fridge)\\
        && move 1 (kitchen)\\
        && finish 0 (floor)\\
        \hline
        \multirow{6}{0.2\textwidth}{Move-LongOpen-Place-Longclose-Move-Finish}
        &\multirow{6}{0.3\textwidth}{Please head to the draw, open it, place the object inside, close it, then proceed to the kitchen.}
        & move 9 (draw)\\
        && longitudinal open 9 (draw)\\
        && place to 9 (draw)\\
        && longitudinal close 9 (draw)\\
        && move 1 (kitchen)\\
        && finish 0 (floor)\\
        \hline
        % Removed task type of length 7
        % \multirow{7}{0.2\textwidth}{move open pick close move place\_to finish}
        % &\multirow{7}{0.3\textwidth}{Please move to the fridge, open it, pick up an tea cup inside, close it, then move to the dining table and place it there.}
        % & move 35 (fridge)\\
        % && revolute open 35 (fridge)\\
        % && pick 45 (tea cup)\\
        % && revolute close 35 (fridge)\\
        % && move 22 (dining table)\\
        % && place to 22 (dining table)\\
        % && finish 0 (floor)\\
        % \hline
	\end{tabular}
    \caption{Instruction-subtask examples.}\label{tab-instruction-subtask-examples}
\end{table*}

==> figure/dataset_statistics/prompt_table.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{|p{0.95\textwidth}|}
        \hline
        \\
        \#Role:
        \\\quad You are an instruction planning model for a mobile grasping robot, your aim is to break down high-level instruction into subtasks for the robot to execute. 
        \\\#Output Restriction: 
        \\\quad Your output is in a form of \textless action\textgreater \textless operating object name\textgreater \textless operating object id\textgreater , where \textless action\textgreater is one of the actions in 
        ['move', 'pick', 'finish', 'place\_to', 'LongOpen', 'LongClose', 'RevOpen', 'RevClose'], 

        The meaning of the actions are:
        \\\quad move: controls the robot movement, the target object is the location where the robot will be moved to.
        \\\quad pick: controls the robot arm, the target object is the object which the robot should pick up.
        \\\quad finish: Showing that the high-level instruction task is completed. The target object does not matter thus the object prediction can be anything.
        \\\quad place\_to: controls the robot arm, the target object is the location where the robot will place the grasping object to.
        \\\quad LongOpen: controls the robot arm to perform a longitudinal open movement on an object, like a sliding drawer or dresser.
        \\\quad LongClose: controls the robot arm to perform a longitudinal close movement on an object, like a sliding drawer or dresser.
        \\\quad RevOpen: controls the robot arm to perform a revolute open movement on an object, like a hinged door or cabinet.
        \\\quad RevClose: controls the robot arm to perform a revolute close movement on an object, like a hinged door or cabinet.

        The \textless operating object name\textgreater  \textless operating object id\textgreater are the object and ids given in the prompt \#Scene.
        Specially, When robot think the task has already reached completion, or the robot should wait for further instruction, output: finish floor 0.

        \\\#Scene:
        \\\quad The current scene has objects with ids: \textless \texttt{scene graph nodes description}\textgreater 
        The relationships between objects in the scenes are: \textless \texttt{scene graph edges description}\textgreater 
        \\\#Robot:
        \\\quad The objects and object ids around the robot are: \textless \texttt{robot graph edges description}\textgreater 
        The relationships between objects around the robot are: \textless \texttt{robot graph edges description}\textgreater 
        \\\#Instruction:
        \textless \texttt{instruction}\textgreater 
        \\\#Task: Please tell me what is the current subtask the robot should perform according to the scene and robot status.
        
        \\\#Example1:
        \\\quad input: 
            \\\quad\#Scene:
            \\\quad\quad The current scene has objects with ids: floor 0, dining room 1, black dining table 2, purple display shelves 3, bathroom 4, brown vanity sink 5
            \\\quad\quad The relationships between objects in the scenes are: dining room 1 is in floor 0, dining table 2 is in dining room 1, display shelves 3 is in dining room 1, bathroom 4 is in floor 0, vanity sink 5 is in bathroom 4
            \\\quad\#Robot:
            \\\quad\quad The objects and object ids around the robot are: robot 0, brown pen 2.
            \\\quad\quad The relationships between objects around the robot are: pen 2 is grasped by robot 0.
            \\\quad\#Instruction:
            Your goal is to get the object to the purple display shelves.
            \\\quad\#Task: Please tell me what is the current subtask the robot should perform according to the scene and robot status.
            \\\quad\#Think: Because I do not know where I am, so I should first move to purple display shelves. So output: move purple display shelves 3.
            
        \\\#Example2:
        \\\quad input: 
            \\\quad\#Scene:
            \\\quad\quad The current scene has objects with ids: floor 0, dining room 1, black dining table 2, purple display shelves 3, bathroom 4, brown vanity sink 5, brown pen 6
            \\\quad\quad The relationships between objects in the scenes are: dining room 1 is in floor 0, dining table 2 is in dining room 1, display shelves 3 is in dining room 1, bathroom 4 is in floor 0, vanity sink 5 is in bathroom 4, brown pen 6 is on display shelves 3
            \\\quad\#Robot:
            \\\quad\quad The objects and object ids around the robot are: robot 0, purple display shelves 3.
            \\\quad\quad The relationships between objects around the robot are: pen 2 is grasped by robot 0.
            \\\quad\#Instruction:
            Your goal is to get the object to the purple display shelves.
            \\\quad\#Task: Please tell me what is the current subtask the robot should perform according to the scene and robot status.
            \\\quad\#Think: Because I no longer have anything grasped in my manipulators, and I am approaching another object, this indicates that I have already completed the instruction to place the object. So output: finish floor 0.

        \\
        \hline
    \end{tabular}
    \caption{The template of prompt and role being sent to ChatGPT4, we fill in the instruction and serialized graph descriptions to get an response from chatGPT4 API.}
    \label{tab-GPT_Prompt}
\end{table*}

